The Biosensor based on electrochemical dynamics of fermentation in yeast Saccharomyces Cerevisiae

The zymase activity of the yeast Saccharomyces Cerevisiae is sensitive to environmental parameters and is therefore used as a microbiological sensor for water quality assessment, ecotoxicological characterization or environmental monitoring. Comparing to bacterial bioluminescence approach, this method has no toxicity, excludes usage of genetically modified microorganisms, and enables low-cost express analysis. This work focuses on measuring the yeast fermentation dynamics based on multichannel pressure sensing and electrochemical impedance spectroscopy (EIS). Measurement results are compared with each other in terms of accuracy, reproducibility and ease of use in the field conditions. It has been shown that EIS provides more information about ionic dynamics of metabolic processes and requires less complex measurements. The conducted experiments demonstrated the sensitivity of this approach for assessing biophotonic phenomena, non-chemical water treatments and impact of environmental stressors.

==> bibliography.tex <==
% Encoding: UTF-8


@article{Goffeau25101996,
author = {Goffeau, A. and Barrell, B. G. and Bussey, H. and Davis, R. W. and Dujon, B. and Feldmann, H. and Galibert, F. and Hoheisel, J. D. and Jacq, C. and Johnston, M. and Louis, E. J. and Mewes, H. W. and Murakami, Y. and Philippsen, P. and Tettelin, H. and Oliver, S. G.},
title = {Life with 6000 Genes},
volume = {274},
number = {5287},
pages = {546-567},
year = {1996},
journal = {Science}
}


@book{Kittel95,
author = {Charles Kittel},
title = {Introduction to Solid State Physics},
publisher = {Wiley \& Sons},
year = {1995}
}




@article {JIB:JIB3223,
author = {Griffin, S. R.},
title = {Maltase activity in {\em saccharomyces cerevisiae} during fermentation of synthetic media},
journal = {Journal of the Institute of Brewing},
volume = {75},
number = {4},
publisher = {Blackwell Publishing Ltd},
pages = {342--346},
year = {1969},
}





@article {JIB:JIB2843,
author = {White, J.},
title = {Enzyme production by yeasts},
journal = {Journal of the Institute of Brewing},
volume = {62},
number = {2},
publisher = {Blackwell Publishing Ltd},
issn = {2050-0416},
pages = {161--169},
year = {1956},
}


@article{Herrera91,
author = {Herrera, V. E.},
title = {Induction of premature yeast flocculation by a polysaccharide fraction isoalted from malt husk},
journal = {J. Inst. Brew.},
volume = {},
number = {97},
pages = {359--366},
year = {1991},
}


@article{Stratford92,
author = {Stratford, M.},
title = {Yeast flocculation: reconciliation of physiological and genetic viewpoints},
journal = {Yeast},
volume = {},
number = {8},
pages = {25--38},
year = {1992},
}


@book{Bobrov01en,
author = {A.V.Bobrov},
title = {Investigation of non-electromagnetic components in emission of quantum generators},
publisher = {VINITI, 2222-B2001},
year = {2001}
}


@INPROCEEDINGS{Bobrov02en,
author={A.V. Bobrov},
booktitle={VINITI N 2282--2002},
title={{B}iological and physical properties of activated water (rus)},
year={2002},
}



@Article{s8106433,
AUTHOR = {V\"alimaa, Anna-Liisa and Kivist\"o, Anniina and Virta, Marko and Karp, Matti},
TITLE = {Real-time Monitoring of Non-specific Toxicity Using a Saccharomyces cerevisiae Reporter System},
JOURNAL = {Sensors},
VOLUME = {8},
YEAR = {2008},
NUMBER = {10},
PAGES = {6433--6447},
URL = {http://www.mdpi.com/1424-8220/8/10/6433},
ISSN = {1424-8220},
ABSTRACT = {Baker's yeast, Saccharomyces cerevisiae, is the simplest and most well-known representative of eukaryotic cells and thus a convenient model organism for evaluating toxic effects in human cells and tissues. Yeast cell sensors are easy to maintain with short generation times, which makes the analytical method of assessing antifungal toxicity cheap and less-time consuming. In this work, the toxicity of test compounds was assessed in bioassays based on bioluminescence inhibition and on traditional growth inhibition on agar plates. The model organism in both tests was a modified S. cerevisiae sensor strain that produces light when provided with D-luciferin in an insect luciferase reporter gene activity assay. The bioluminescence assay showed toxic effects for yeast cell sensor of 5,6-benzo-flavone, rapamycin, nystatin and cycloheximide at concentrations of nM to �M. In addition, arsenic compounds, cadmium chloride, copper sulfate and lead acetate were shown to be potent non-specific inhibitors of the reporter organism described here. The results from a yeast agar diffusion assay correlated with the bioluminescence assay results.},
DOI = {10.3390/s8106433}
}


@article{Gromozova15,
author = {Gromozova E.N. and Kachur T.L. and Voychuk S.I. and Kharchuk M.S.},
title = {The reaction of phosphorus-containing intracellular inclusions to space weather changes},
journal = {Odessa Astronomical Publications},
volume = {28},
number = {2},
pages = {261--263},
year = {2015},
}



@inproceedings{doi:10.1117/12.2017989,
author = {Rogacheva, Svetlana M. and Babaeva, Milena I.},
title = {The effect of millimeter waves at the yeast Saccharomyces cerevisiae during heliogeophysical disturbances},
booktitle = {Proc. SPIE},
volume = {8699},
number = {},
pages = {86990N-86990N-7},
abstract = {The isolated and combined effect of heliogeophysical factors and low intensive electromagnetic radiation of millimeter diapason at the metachromasia reaction of the yeast Saccharomyces cerevisiae was studied. It was established that longterm influence of EMR 65 GHz induced changes in the response of cells towards heliogeomagnetic disturbance. On our opinion millimeter waves may reduce the effect of heliogeophysical factors on living organisms because of  destabilization of the intracellular water structure.},
year = {2013},
doi = {10.1117/12.2017989},
URL = {http://dx.doi.org/10.1117/12.2017989},
}

@InProceedings{Bobrov2002,
  author    = {A.V. Bobrov},
  title     = {{B}iological and physical properties of activated water (rus)},
  booktitle = {VINITI N 2282-�2002},
  year      = {2002},
}


@INPROCEEDINGS{Gorshkov72,
author = {Gorshkov, M.M. and Davidov, M.G.},
title = {The {C}hizhevsky-{V}elhover effect},
booktitle = {Sun. Electrocity, Life (rus)},
publisher = {Moscow, MGU, 52-54},
year = {1972}
}






@ARTICLE{Kernbach14Biominimalen,
  author = {S.Kernbach},
  title = {Minimal microbiological experiment (rus)},
  journal = {International Journal of Uncoventional Science},
  pages = {45--54},
  volume = {6},
  number = {2},
  year = {2014},
}



@article {JIB:JIB2789,
author = {White, J. and Munns, D. J.},
title = {Some aspects of osmosensitivity in yeasts: i. significance and measurement of osmosensitivity},
journal = {Journal of the Institute of Brewing},
volume = {61},
number = {3},
publisher = {Blackwell Publishing Ltd},
issn = {2050-0416},
pages = {217--223},
year = {1955},
}


@book{ANKOM17,
author = {ANKOM},
title = {ANKOM RF Gas Production Measurement System},
publisher = {Specification document, www.ankom.com},
year = {2017}
}


@article{Nealson79,
author = {Nealson K.H. and Hastings J.W.},
title = {Bacterial bioluminescence: its control and ecological significance},
journal = {Microbiological Reviews},
volume = {43},
number = {4},
pages = {496-518},
year = {1979},
}


@article{Ritchie01062003,
author = {Ritchie, Jennifer M. and Campbell, Graeme R. and Shepherd, Jill and Beaton, Yvonne and Jones, Davey and Killham, Ken and Artz, Rebekka R. E.},
title = {A Stable Bioluminescent Construct of Escherichia coli O157:H7 for Hazard Assessments of Long-Term Survival in the Environment},
volume = {69},
number = {6},
pages = {3359-3367},
year = {2003},
journal = {Applied and Environmental Microbiology}
}


@inproceedings{Rampl2009,
 author = {Rampl, Ivan and Boudn\'{y}, Vladim\'{\i}r and C\'{\i}\v{z}, Milan and Lojek, Anton\'{\i}n and Hyr\v{s}l, Pavel},
 title = {Pulse Vector Magnetic Potential and Its Influence on Live Cells},
 booktitle = {Proceedings of the 2009 International Conference on eHealth, Telemedicine, and Social Medicine},
 series = {ETELEMED '09},
 year = {2009},
 isbn = {978-0-7695-3532-6},
 pages = {99--107},
 numpages = {9},
 doi = {10.1109/eTELEMED.2009.47},
 acmid = {1510625},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {magnetic field, pulse vector magnetic potential, toroidal coil, cell metabolism, chemiluminescence, bioluminescence, oncogenically transformed cells, human malignant melanoma, breast carcinoma},
}


@article{Anosov03en,
author = {V.N. Anosov and E.M. Truchan},
title = {New approach to impact of weak magnetic fields on living objects (rus)},
journal = {{Doklady Akedemii Nauk}: biochemistry, biophysics and molecular biology},
number = {392},
pages = {1-5},
year = {2003}
}

\
@article{NUNES-HALLDORSON2003,
   title = {{Bioluminescent bacteria: lux genes as environmental biosensors}},
   journal = {{Brazilian Journal of Microbiology}},
   author={Nunes-Halldorson, V\^ania da Silva AND Duran, Norma Let\'icia},
   ISSN = {1517-8382},
   language = {en},
   volume = {34},
   year = {2003},
   month = {06},
   pages = {91--96},
   publisher = {scielo},
   }


@Article{Palmer2006,
author="Palmer, S. J.
and Rycroft, M. J.
and Cermack, M.",
title="Solar and geomagnetic activity, extremely low frequency magnetic and electric fields and human health at the Earth's surface",
journal="Surveys in Geophysics",
year="2006",
month="Sep",
day="01",
volume="27",
number="5",
pages="557--595",
abstract="The possibility that conditions on the Sun and in the Earth's magnetosphere can affect human health at the Earth's surface has been debated for many decades. This work reviews the research undertaken in the field of heliobiology, focusing on the effect of variations of geomagnetic activity on human cardiovascular health. Data from previous research are analysed for their statistical significance, resulting in support for some studies and the undermining of others. Three conclusions are that geomagnetic effects are more pronounced at higher magnetic latitudes, that extremely high as well as extremely low values of geomagnetic activity seem to have adverse health effects and that a subset of the population (10--15{\%}) is predisposed to adverse health due to geomagnetic variations. The reported health effects of anthropogenic sources of electric and magnetic fields are also briefly discussed, as research performed in this area could help to explain the results from studies into natural electric and magnetic field interactions with the human body.",
issn="1573-0956",
doi="10.1007/s10712-006-9010-7",
url="http://dx.doi.org/10.1007/s10712-006-9010-7"
}


@book{konig2012biologic,
  title={Biologic Effects of Environmental Electromagnetism},
  author={K{\"o}nig, H.L. and Telger, T.C. and Kr{\"u}ger, A.P. and Lang, S. and S{\"o}nning, W.},
  isbn={9781461258599},
  series={Topics in Environmental Physiology and Medicine},
  url={https://books.google.de/books?id=IIjTBwAAQBAJ},
  year={2012},
  publisher={Springer New York}
}



@book{Chizhevsky36,
author = {Alexander Chizhevsky},
title = {The Terrestrial Echo of Solar Storms},
publisher = {Moscow},
year = {1936}
}


@book{ABER17,
author = {ABER instruments},
title = {Compact Yeast Monitor},
publisher = {Specification document, www.aberinstruments.com},
year = {2017}
}


@book{campbell2012sensor,
  title={Sensor Systems for Environmental Monitoring: Volume One: Sensor Technologies},
  author={Campbell, M.},
  isbn={9789400915718},
  url={https://books.google.de/books?id=EtLsCAAAQBAJ},
  year={2012},
  publisher={Springer Netherlands}
}


@article{doi:10.1021/jf9911794,
author = {Kurittu, Jussi and L\"onnberg, Stefan and Virta, Marko and Karp, Matti},
title = {A Group-Specific Microbiological Test for the Detection of Tetracycline Residues in Raw Milk},
journal = {Journal of Agricultural and Food Chemistry},
volume = {48},
number = {8},
pages = {3372-3377},
year = {2000}
}


@article{Deryabin04,
author = {D.G. Deryabin and E.G. Polyakov},
title = {Effect of Human Serum on Bioluminescence of Natural and Recombinant Luminescent Bacteria},
journal = {Bulletin of Experimental Biology and Medicine},
volume = {138},
number = {9},
pages = {3372-3377},
year = {2004}
}

@BOOK{Kernbach15en,
  author = {S. Kernbach},
  title = {Supernatural. Scientifically proven facts},
  publisher = {Algorithm. Moscow},
  year = {2015},
}


@ARTICLE{Kernbach12JSE,
  author = {Serge Kernbach},
  title = {Replication Attempt: Measuring Water Conductivity with Polarized Electrodes},
  journal = {Journal of Scientific Exploration},
  pages = {69--105},
  volume = {27},
  number = {1},
  year = {2013},
}

@article{Puthoff98,
author = {H.E. Puthoff},
title = {Communication Method and Apparatus with Signals Comprising Scalar and Vector Potentials without Electromagnetic Fields},
journal = {Patent US5845220},
number = {},
pages = {},
year = {1998}
}


@article{Aharonov59,
    author = {Aharonov, Y. and Bohm, D.},
    journal = {Physical Review Online Archive (Prola)},
    number = {3},
    pages = {485--491},
    publisher = {American Physical Society},
    title = {{Significance of Electromagnetic Potentials in the Quantum Theory}},
    volume = {115},
    year = {1959}
}


@article{PANDARD2006114,
title = "Selecting a battery of bioassays for ecotoxicological characterization of wastes",
journal = "Science of The Total Environment",
volume = "363",
number = "1",
pages = "114 - 125",
year = "2006",
note = "",
issn = "0048-9697",
doi = "http://dx.doi.org/10.1016/j.scitotenv.2005.12.016",
url = "http://www.sciencedirect.com/science/article/pii/S0048969705009216",
author = "Pascal Pandard and James Devillers and Anne-Marie Charissou and Véronique Poulsen and Marie-José Jourdain and Jean-François Férard and Cécile Grand and Antonio Bispo",
keywords = "Ecotoxicity",
keywords = "Bioassay",
keywords = "Waste",
keywords = "Hazard",
keywords = "Test battery",
keywords = "Multivariate analyses"
}


@article{ROJICKOVAPADRTOVA1998495,
title = "Evaluation of alternative and standard toxicity assays for screening of environmental samples: Selection of an optimal test battery",
journal = "Chemosphere",
volume = "37",
number = "3",
pages = "495 - 507",
year = "1998",
note = "",
issn = "0045-6535",
doi = "http://dx.doi.org/10.1016/S0045-6535(98)00065-4",
url = "http://www.sciencedirect.com/science/article/pii/S0045653598000654",
author = "Renata Roj\`i\v{c}kov\`a-Padrtov\`a and Blahoslav Mar\v{s}lek and Ivan Holoubek",
keywords = "alternative assay",
keywords = "microbiotest",
keywords = "standard toxicity test",
keywords = "environmental sample",
keywords = "sensitivity",
keywords = "acute toxicity",
abstract = "Six muniaturized alternative assays (called microbiotests) and three standard toxicity tests were used for a comparative study based on the evaluation of acute toxicity of fifty environmental samples. The test species used in the alternative assays were microalga Raphidocelis subcapitata, crustaceans Thamnocephalus platyurus and Ceriodaphnia dubia, rotifer Brachionus calyciflorus,protozoan Spirostomum ambiguum and bacterium Vibrio fischeri. The standard toxicity tests utilized microalga Raphidocelis subcapitata, crustacean Daphnia magna, and fish Poecilia reticulata as the test organisms. The study compared the ability of bioassays to detect acute toxicity, relative sensitivity of the six microbiotests with regard to three standard toxicity tests, and similarity in their sensitivity to fifty samples. Algal bioassays were the most sensitive tests. Ceriodaphnia dubia and Spirostomum ambiguum detected acute toxicity in the majority of samples (in 62–72%). Vibrio fischeri showed a specific sensitivity pattern that was associated neither with algal nor with animal tests. The other species formed the least sensitive organisms, having similar sensitivities. A battery of three to four alternative assays was selected on the basis of the statistical analyses, sensitivity comparisons and general conditions for the selection of a test battery member like incorporation of different trophic levels or complementation of assays in a battery. Therefore, miniaturized algal assay, rotifer or crustacean microbiotest, bacterial test and possibly protozoan microbiotest could represent an optimal battery of alternative asaays for the toxicity evaluation of fifty environmental samples presented in this study."
}




@article{KARUBE198869,
title = "Application of microbiological sensors in fermentation processes",
journal = "Analytica Chimica Acta",
volume = "213",
number = "",
pages = "69 - 77",
year = "1988",
note = "",
issn = "0003-2670",
doi = "http://dx.doi.org/10.1016/S0003-2670(00)81341-0",
url = "http://www.sciencedirect.com/science/article/pii/S0003267000813410",
author = "Isao Karube and Eiichi Tamiya and Koji Sode and Kenji Yokoyama and Yasushi Kitagawa and Hiroaki Suzuki and Yasukasu Asano",

}


@inproceedings{voeikov2006,
    author = "Voeikov, V.L.",
		editor = "BlaBlau, V.L.",
    title = "Fundamental Role of Water in Bioenergetics",
    booktitle = "Biophotonics and Coherent Systems in Biology. L.V. Beloussov, V.L. Voeikov, V.S. Martynyuk, (eds.)",
    year = "2006",
    pages = "89--104",
    publisher = "Springer"
}

@Article{Kim2003,
author="Kim, Byung Hong
and Chang, In Seop
and Cheol Gil, Geun
and Park, Hyung Soo
and Kim, Hyung Joo",
title="Novel BOD (biological oxygen demand) sensor using mediator-less microbial fuel cell",
journal="Biotechnology Letters",
year="2003",
month="Apr",
day="01",
volume="25",
number="7",
pages="541--545",
abstract="A microbial fuel cell type of biosensor was used to determine the biochemical oxygen demand (BOD) of wastewater. The biosensor gave a good correlation between the BOD value and the coulomb produced. The BOD sensor has been operated for over 5 years in a stable manner without any servicing. This is much longer that that of previously reported BOD biosensors.",
issn="1573-6776",
doi="10.1023/A:1022891231369",
url="http://dx.doi.org/10.1023/A:1022891231369"
}


@incollection{bath50782,
           month = {December},
          author = {M. Di Lorenzo},
          series = {Woodhead Publishing Series in Energy},
       booktitle = {Microbial Electrochemical and Fuel Cells},
          editor = {K. Scott and E. Hao Yu},
           title = {Use of microbial fuel cells in sensors},
         address = {Cambridge, U. K.},
       publisher = {Woodhead Publishing},
            year = {2015},
           pages = {341--356},
        keywords = {bioactive toxicants,biosensors,bod,cod,microbial fuel cell,micropollutants},
             url = {http://opus.bath.ac.uk/50782/},
        abstract = {This chapter reviews the state-of-the-art use of microbial fuel cells (MFCs) as sensors for the online monitoring of water quality. This is a very promising application of MFC technology that has not yet been fully explored. The most intuitive analytical application of MFCs is with regards to the monitoring of the labile organic carbon content in wastewaters. This is because, within a specific range dictated by the Monod equation, the amount of electrons produced by the anode biofilm is a direct function of the concentration of biodegradable organic compounds in the feeding water. The literature on the use of MFCs as a tool to measure the chemical and biological oxygen demand in wastewaters is therefore well established and includes also in-field validations.Much more recently, there has been an increasing interest in exploring the use of MFCs also as a means to detect toxicants in water, which is encouraged by the great advantages of this technology over traditional analytical methodologies. MFCs can in fact operate in the field and online and have the great benefits of simplicity, higher stability compared to enzyme-based sensors, and depending on the material used, cost-effectiveness. The very few proof-of-concept studies on this topic are very promising. The presence of a bioactive toxicant in the feed affects the performance of the electroactive biofilm at the anode and causes a change in the MFC outputs that is easily detected. The full possibilities that MFCs open in the field of water quality monitoring have to be, however, better explored. In particular, some challenges, such as sensitivity and selectivity, remain still to be addressed.},
             doi = {10.1016/B978-1-78242-375-1.00011-3}
}



@Article{bios5030450,
AUTHOR = {Chouler, Jon and Di Lorenzo, Mirella},
TITLE = {Water Quality Monitoring in Developing Countries;  Can Microbial Fuel Cells be the Answer?},
JOURNAL = {Biosensors},
VOLUME = {5},
YEAR = {2015},
NUMBER = {3},
PAGES = {450--470},
URL = {http://www.mdpi.com/2079-6374/5/3/450},
ISSN = {2079-6374},
ABSTRACT = {The provision of safe water and adequate sanitation in developing countries is a must. A range of chemical and biological methods are currently used to ensure the safety of water for consumption. These methods however suffer from high costs, complexity of use and inability to function onsite and in real time. The microbial fuel cell (MFC) technology has great potential for the rapid and simple testing of the quality of water sources. MFCs have the advantages of high simplicity and possibility for onsite and real time monitoring. Depending on the choice of manufacturing materials, this technology  can also be highly cost effective. This review covers the state-of-the-art research on  MFC sensors for water quality monitoring, and explores enabling factors for their use in developing countries.},
DOI = {10.3390/bios5030450}
}

@Manual{Honeywell2015,
  title  = {Miniature Low Pressure Sensors 26PC Series, Compensated/Unamplified},
  author = {Honeywell},
  year   = {2015},
  url    = {https://sensing.honeywell.com/index.php?ci_id=155865},
}

@Manual{Instruments2015,
  title  = {INA333 Micro-Power, Zero-Drift, Rail-to-Rail Out Instrumentation Amplifier},
  author = {Texas Instruments},
  year   = {2015},
  url    = {http://www.ti.com/lit/ds/symlink/ina333.pdf},
}

@Manual{ST2017,
  title  = {LDLN015 ultra low noise linear voltage regulator IC},
  author = {ST},
  year   = {2017},
  url    = {http://www.st.com/content/ccc/resource/technical/document/datasheet/9d/4b/35/ac/73/9e/4b/69/DM00047215.pdf/files/DM00047215.pdf/jcr:content/translations/en.DM00047215.pdf},
}

@Manual{Instruments2016,
  title  = {LM4140 High Precision Low Noise Low Dropout Voltage Reference},
  author = {Texas Instruments},
  year   = {2016},
  url    = {http://www.ti.com/lit/ds/symlink/lm4140.pdf},
}

@Manual{Cypress2017,
  title  = {PSoC 5LP: CY8C58LP Family Datasheet},
  author = {Cypress},
  year   = {2017},
  url    = {http://www.cypress.com/file/45906/download},
}

@book{prasad2004introduction,
  title={Introduction to Biophotonics},
  author={Prasad, P.N.},
  isbn={9780471465393},
  url={https://books.google.it/books?id=zF1GYVamV34C},
  year={2004},
  publisher={Wiley}
}



@book{Harfst10,
  title={Non-chemical water treatment},
  author={W.R. Harfst},
  year={2010},
  publisher={Chem. Eng. (April 2010), pp. 66-69}
}


@article{PIYADASA201719,
title = "The application of electromagnetic fields to the control of the scaling and biofouling of reverse osmosis membranes - A review",
journal = "Desalination",
volume = "418",
number = "Supplement C",
pages = "19 - 34",
year = "2017",
issn = "0011-9164",
doi = "https://doi.org/10.1016/j.desal.2017.05.017",
url = "http://www.sciencedirect.com/science/article/pii/S0011916416317829",
author = "Chathuri Piyadasa and Harry F. Ridgway and Thomas R. Yeager and Matthew B. Stewart and Con Pelekani and Stephen R. Gray and John D. Orbell",
keywords = "Scaling, Biofouling, Cleaning, Pulsed electric fields, Electromagnetic fields"
}



@article{doi:10.1021/ja972171i,
author = {Suslick, Kenneth S. and Mdleleni, Millan M. and Ries, Jeffrey T.},
title = {Chemistry Induced by Hydrodynamic Cavitation},
journal = {Journal of the American Chemical Society},
volume = {119},
number = {39},
pages = {9303-9304},
year = {1997},
doi = {10.1021/ja972171i},
}

@article{ALIMI20091327,
title = "Effect of magnetic water treatment on calcium carbonate precipitation: Influence of the pipe material",
journal = "Chemical Engineering and Processing: Process Intensification",
volume = "48",
number = "8",
pages = "1327 - 1332",
year = "2009",
issn = "0255-2701",
doi = "https://doi.org/10.1016/j.cep.2009.06.008",
url = "http://www.sciencedirect.com/science/article/pii/S0255270109000956",
author = "F. Alimi and M.M. Tlili and M. Ben Amor and G. Maurin and C. Gabrielli",
keywords = "Magnetic field",
keywords = "Calcium carbonate",
keywords = "Scaling",
keywords = "Hard water",
keywords = "Pipe material"
}

@InProceedings{Rampl2009a,
  author    = {Rampl, Ivan and Boudn\'{y}, Vladim\'{\i}r and C\'{\i}\v{z}, Milan and Lojek, Anton\'{\i}n and Hyr\v{s}l, Pavel},
  title     = {Pulse Vector Magnetic Potential and Its Influence on Live Cells},
  booktitle = {Proceedings of the 2009 International Conference on eHealth, Telemedicine, and Social Medicine},
  year      = {2009},
  series    = {ETELEMED '09},
  pages     = {99--107},
  address   = {Washington, DC, USA},
  publisher = {IEEE Computer Society},
  acmid     = {1510625},
  doi       = {10.1109/eTELEMED.2009.47},
  isbn      = {978-0-7695-3532-6},
  keywords  = {magnetic field, pulse vector magnetic potential, toroidal coil, cell metabolism, chemiluminescence, bioluminescence, oncogenically transformed cells, human malignant melanoma, breast carcinoma},
  numpages  = {9},
}


@ARTICLE{Kernbach17water,
  author = {S. Kernbach and I. Kuksin and O. Kernbach},
  title = {On Accurate Differential Measurements with Electrochemical Impedance Spectroscopy},
  journal = {WATER},
  pages = {136-155},
  volume = {8},
  number = {},
  year = {2017},
}


@ARTICLE{Kernbach17EISen,
  author = {S.Kernbach and O.Kernbach},
  title = {Reliable detection of weak emissions by the {EIS} approach},
  journal = {IJUS},
  pages = {65-79},
  volume = {14},
  number = {4},
  year = {2017},
}



@Article{s150922941,
AUTHOR = {Conesa, Claudia and Garcia-Breijo, Eduardo and Loeff, Edwin and Segui, Lucia and Fito, Pedro and Laguarda-Miro, Nicolas},
TITLE = {An Electrochemical Impedance Spectroscopy-Based Technique to Identify and Quantify Fermentable Sugars in Pineapple Waste Valorization for Bioethanol Production},
JOURNAL = {Sensors},
VOLUME = {15},
YEAR = {2015},
NUMBER = {9},
PAGES = {22941--22955},
}


@article{JEB664,
	author = {Martin Zamora and Gabriel Ruiz and Carmelo Felice},
	title = {Evaluation of sugar yeast consumption by measuring electrical medium resistance},
	journal = {Journal of Electrical Bioimpedance},
	volume = {4},
	number = {1},
	year = {2013},
	keywords = {Yeast;sugar consumption; monitoring; CO2; medium resistance},
	abstract = {The real-time monitoring of alcoholic fermentation (sugar consumption) is very important in industrial processes. Several techniques (i.e., using a biosensor) have been proposed to realize this goal. In this work, we propose a new method to follow sugar yeast consumption. This novel method is based on the changes in the medium resistance (Rm) that are induced by the CO2 bubbles produced during a fermentative process. We applied a 50-mV and 700-Hz signal to 75 ml of a yeast suspension in a tripolar cell. A gold electrode was used as the working electrode, whereas an Ag/AgCl electrode and a stainless-steel electrode served as the reference and counter electrodes, respectively. We then added glucose to the yeast suspension and obtained a 700% increase in the Rm after 8 minutes. The addition of sucrose instead of glucose as the carbon source resulted in a 1200% increase in the Rm. To confirm that these changes are the result of CO2 bubbles in the fermentation medium, we designed a tetrapolar cell in which CO2 gas was insufflated at the bottom of the cell and concluded that the changes were due to CO2 bubbles produced during the fermentation. Consequently, this new method is a low-cost and rapid technology to follow the sugar consumption in yeast.},
	issn = {1891-5469},	url = {https://www.journals.uio.no/index.php/bioimpedance/article/view/664}
}



@ARTICLE{Kernbach17Verdyen,
  author = {S. Kernbach and I.Kuksin and O.Kernbach and A.Kernbach},
  title = {The Vernadsky scale -- on metrology of {EIS} in time-frequency domain},
  journal = {IJUS},
  pages = {62-87},
  volume = {143--150},
  number = {5},
  year = {2017},
}


@book{dickinson2004metabolism,
  title={Metabolism and Molecular Physiology of Saccharomyces Cerevisiae, 2nd Edition},
  author={Dickinson, J.R. and Schweizer, M.},
  isbn={9780203503867},
  lccn={2003060837},
  url={https://books.google.de/books?id=yPKOT4NmHUkC},
  year={2004},
  publisher={CRC Press}
}


@ARTICLE{Kernbach13arXiv,
   author = {{Kernbach}, S.},
   title = "{Unconventional research in USSR and Russia: short overview}",
   journal = {arXiv 1312.1148},
   year = 2013,
   adsurl = {http://adsabs.harvard.edu/abs/2013arXiv1312.1148K},
}


@article{Popp94,
author = {Popp, Fritz-Albert and Gu, Qiao and Li, Ke-Hsueh},
title = {Biophoton Emission: Experimental Background and Theoretical Approaches},
journal = {Modern Physics Letters B},
volume = {08},
number = {21n22},
pages = {1269-1296},
year = {1994},
doi = {10.1142/S0217984994001266},
}


@book{Gurvich44en,
author = {A.G.Gurvich},
title = {Theory of biological fields (rus)},
publisher = {M.: Soviet science},
year = {1944},
}


@book{Kaznacheev81en,
author = {V.P. Kaznacheev and L.P. Michailova},
title = {Ultraweak emissions in intercellular interactions (rus)},
publisher = {Hauka},
year = {1981}
}

@Article{Slouka2017,
  author    = {Christoph Slouka and Georg Brunauer and Julian Kopp and Michael Strahammer and Jens Fricke and Jürgen Fleig and Christoph Herwig},
  title     = {Low-Frequency Electrochemical Impedance Spectroscopy as a Monitoring Tool for Yeast Growth in Industrial Brewing Processes},
  journal   = {Chemosensors},
  year      = {2017},
  volume    = {5},
  number    = {3},
  pages     = {24},
  month     = {aug},
  doi       = {10.3390/chemosensors5030024},
  publisher = {{MDPI} {AG}},
}

@Article{Soley2005,
  author    = {A. Soley and M. Lecina and X. G{\'{a}}mez and J.J. Cair{\'{o}} and P. Riu and X. Rosell and R. Brag{\'{o}}s and F. G{\`{o}}dia},
  title     = {On-line monitoring of yeast cell growth by impedance spectroscopy},
  journal   = {Journal of Biotechnology},
  year      = {2005},
  volume    = {118},
  number    = {4},
  pages     = {398--405},
  month     = {sep},
  doi       = {10.1016/j.jbiotec.2005.05.022},
  publisher = {Elsevier {BV}},
}

@Article{Ebina1989,
  author    = {Y. Ebina and M. Ekida and H. Hashimoto},
  title     = {Origin of changes in electrical impedance during the growth and fermentation process of yeast in batch culture},
  journal   = {Biotechnology and Bioengineering},
  year      = {1989},
  volume    = {33},
  number    = {10},
  pages     = {1290--1295},
  month     = {apr},
  doi       = {10.1002/bit.260331010},
  publisher = {Wiley-Blackwell},
}

@Article{Yardley2000,
  author    = {John E. Yardley and Douglas B. Kell and John Barrett and Christopher L. Davey},
  title     = {On-Line, Real-Time Measurements of Cellular Biomass using Dielectric Spectroscopy},
  journal   = {Biotechnology and Genetic Engineering Reviews},
  year      = {2000},
  volume    = {17},
  number    = {1},
  pages     = {3--36},
  month     = {aug},
  doi       = {10.1080/02648725.2000.10647986},
  publisher = {Informa {UK} Limited},
}



@INPROCEEDINGS{Kornienko_S03A,
  author = {S.~Kornienko and O.~Kornienko and P.~Levi},
  title = {Flexible manufacturing process planning based on the multi-agent
	technology},
  booktitle = {Proc. of the 21st IASTED Int. Conf. on AI and Applications (AIA '2003),
	Innsbruck, Austria},
  year = {2003},
  pages = {156-161}
}


@INPROCEEDINGS{Kornienko_S04,
  author = {S.~Kornienko and O.~Kornienko and P.~Levi},
  title = {Multi-agent repairer of damaged process plans in manufacturing environment},
  booktitle = {Proc. of the 8th Conf. on Intelligent Autonomous Systems (IAS-8),
	Amsterdam, NL},
  year = {2004},
  pages = {485-494}
}



@INCOLLECTION{Kernbach08online,
  author = {L. K{\"o}nig and K. Jebens and Serge Kernbach and Paul Levi},
  title = {Stability of On-Line and On-Board Evolving of Adaptive Collective Behavior},
  booktitle = {European Robotics Symposium 2008},
  year = {2008},
  editor = {Herman Bruyninckx and Libor Preucil and Miroslav Kulich},
  pages = {293-302},
  doi = {http://dx.doi.org/10.1007/978-3-540-78317-6_30}
}


@INPROCEEDINGS{Kornienko_S05e,
  author = {S. Kornienko and O. Kornienko and P. Levi},
  title = {Swarm embodiment - a new way for deriving emergent behaviour in artificial
	swarms},
  booktitle = {Autonome Mobile Systeme (AMS'05)},
  year = {2005},
  editor = {P.Levi and et al.},
  pages = {25-32},
  ee = {http://dx.doi.org/10.1007/3-540-30292-1_4}
}


@INPROCEEDINGS{Thenius16,
  author = {Thenius, R. and et al.},
  title = {subCULTron – Cultural development as tool in underwater robotics},
  booktitle = {Artificial Life and Intelligent Agents Symposium},
  year = {2016}
}

@Article{Male1999,
  author    = {Tone Male and Jens Feder and Guri N. Giaever and Ivar Giaever},
  title     = {Oscillations in Yeast Observed Electrically},
  journal   = {Biological Rhythm Research},
  year      = {1999},
  volume    = {30},
  number    = {4},
  pages     = {361--370},
  month     = {oct},
  doi       = {10.1076/brhm.30.4.361.1411},
  publisher = {Informa {UK} Limited},
}

@Article{Madsen2005,
  author    = {Mads F. Madsen and Sune Dan{\o} and Preben G S{\o}rensen},
  title     = {On the mechanisms of glycolytic oscillations in yeast},
  journal   = {{FEBS} Journal},
  year      = {2005},
  volume    = {272},
  number    = {11},
  pages     = {2648--2660},
  month     = {may},
  doi       = {10.1111/j.1742-4658.2005.04639.x},
  publisher = {Wiley-Blackwell},
}

@Article{Bier2000,
  author    = {Martin Bier and Barbara M. Bakker and Hans V. Westerhoff},
  title     = {How Yeast Cells Synchronize their Glycolytic Oscillations: A Perturbation Analytic Treatment},
  journal   = {Biophysical Journal},
  year      = {2000},
  volume    = {78},
  number    = {3},
  pages     = {1087--1093},
  month     = {mar},
  doi       = {10.1016/s0006-3495(00)76667-7},
  publisher = {Elsevier {BV}},
}

@Book{Alberts2002,
  title     = {Molecular Biology of the Cell, Fourth Edition},
  publisher = {Garland Science},
  year      = {2002},
  author    = {Bruce Alberts and Alexander Johnson and Julian Lewis and Martin Raff and Keith Roberts and Peter Walter},
  isbn      = {0-8153-3218-1},
  url       = {https://www.amazon.com/Molecular-Biology-Fourth-Bruce-Alberts/dp/0815332181?SubscriptionId=0JYN1NVW651KCA56C102&tag=techkie-20&linkCode=xm2&camp=2025&creative=165953&creativeASIN=0815332181},
}

@Article{Chance1964,
  author    = {B. Chance and R. W. Estabrook and A. Ghosh},
  title     = {{DAMPED} {SINUSOIDAL} {OSCILLATIONS} {OF} {CYTOPLASMIC} {REDUCED} {PYRIDINE} {NUCLEOTIDE} {IN} {YEAST} {CELLS}},
  journal   = {Proceedings of the National Academy of Sciences},
  year      = {1964},
  volume    = {51},
  number    = {6},
  pages     = {1244--1251},
  month     = {jun},
  doi       = {10.1073/pnas.51.6.1244},
  publisher = {Proceedings of the National Academy of Sciences},
}

@Article{Laxman2010,
  author    = {Sunil Laxman and Benjamin P Tu},
  title     = {Systems approaches for the study of metabolic cycles in yeast},
  journal   = {Current Opinion in Genetics {\&} Development},
  year      = {2010},
  volume    = {20},
  number    = {6},
  pages     = {599--604},
  month     = {dec},
  doi       = {10.1016/j.gde.2010.09.008},
  publisher = {Elsevier {BV}},
}

@Article{Richard2003,
  author    = {Peter Richard},
  title     = {The rhythm of yeast},
  journal   = {{FEMS} Microbiology Reviews},
  year      = {2003},
  volume    = {27},
  number    = {4},
  pages     = {547--557},
  month     = {oct},
  doi       = {10.1016/s0168-6445(03)00065-2},
  publisher = {Oxford University Press ({OUP})},
}


@Article{Ives14,
  author    = {Ives, JA and van Wijk, EPA and Bat, N and et al.},
  title     = {Ultraweak Photon Emission as a Non-Invasive Health Assessment: A Systematic Review},
  journal   = {{PLoS ONE}},
  year      = {2014},
  volume    = {9},
  number    = {2},
  pages     = {e87401}
}

@article{MASLANKA201855,
title = "Autofluorescence of yeast Saccharomyces cerevisiae cells caused by glucose metabolism products and its methodological implications",
journal = "Journal of Microbiological Methods",
volume = "146",
pages = "55 - 60",
year = "2018",
issn = "0167-7012",
doi = "https://doi.org/10.1016/j.mimet.2018.01.017",
url = "http://www.sciencedirect.com/science/article/pii/S0167701218300514",
author = "Roman Maslanka and Magdalena Kwolek-Mirek and Renata Zadrag-Tecza",
keywords = "Autofluorescence, Endogenous fluorophores, Carbon flow, Glucose analogue, "
}

@book{gikonyo2016advances,
  title={Advances in Biofuel Production: Algae and Aquatic Plants},
  author={Gikonyo, B.},
  isbn={9781482232769},
  lccn={2013949391},
  series={EBL ebooks online},
  url={https://books.google.de/books?id=XC6sCQAAQBAJ},
  year={2016},
  publisher={Apple Academic Press}
}


@Article{Musumeci99,
  author    = {Musumeci, F. and Scordino, A. and Triglia, A. and Blandino, G. and Milazzo, I.},
  title     = {Intercellular communication during yeast cell growth},
  journal   = {Europhys. Lett.},
  year      = {1999},
  volume    = {47},
  number    = {},
  pages     = {736--742}
}


@Article{Hunt09,
  author    = {Hunt, R.W. and Zavalin, A. and Bhatnagar, A. and Chinnasamy, S. and Das, K.C.},
  title     = {Electromagnetic Biostimulation of Living Cultures for Biotechnology, Biofuel and Bioenergy Applications},
  journal   = {International Journal of Molecular Sciences},
  year      = {2009},
  volume    = {10},
  number    = {10},
  pages     = {4515--4558}
}

@Article{JONES1970,
  author    = {R. C. JONES and J. S. HOUGH},
  title     = {The Effect of Temperature on the Metabolism of Baker's Yeast growing on Continuous Culture},
  journal   = {Journal of General Microbiology},
  year      = {1970},
  volume    = {60},
  number    = {1},
  pages     = {107--116},
  month     = {jan},
  doi       = {10.1099/00221287-60-1-107},
  publisher = {Microbiology Society},
}

@Article{Light2005,
  author    = {Truman S. Light and Stuart Licht and Anthony C. Bevilacqua and Kenneth R. Morash},
  title     = {The Fundamental Conductivity and Resistivity of Water},
  journal   = {Electrochemical and Solid-State Letters},
  year      = {2005},
  volume    = {8},
  number    = {1},
  pages     = {E16},
  doi       = {10.1149/1.1836121},
  publisher = {The Electrochemical Society},
}

@Article{Rampl2012,
  author    = {Ivan Rampl and Luk{\'{a}}{\v{s}} Palko and Pavel Hyr{\v{s}}l and Libor Vojtek},
  title     = {Pulsed Vector Magnetic Potential Field Existence},
  journal   = {World Journal of Condensed Matter Physics},
  year      = {2012},
  volume    = {02},
  number    = {04},
  pages     = {202--207},
  doi       = {10.4236/wjcmp.2012.24034},
  publisher = {Scientific Research Publishing, Inc,},
}

@Comment{jabref-meta: databaseType:bibtex;}

%author = {Ronald Thenius and Daniel Moser and Serge Kernbach and Igor Kuksin and Olga Kernbach and Elena Kuksina and Nikola Mišković and Stjepan Bogdan and Tamara Petrović and Anja Babić and Frederic Boyer and Vincent Lebastard and Stephane Bazeille and Graziano William Ferrari and Elisa Donati and Riccardo Pelliccia and Donato Romano and Cesare Stefanini and Matteo Morgantin and Alexandre Campo and Thomas Schmickl},

